HiSC4D: Human-centered interaction and 4D Scene Capture in Large-scale Space Using Wearable IMUs and LiDAR

We introduce HiSC4D, a novel Human-centered interaction and 4D Scene Capture method, aimed at accurately and efficiently creating a dynamic digital world, containing large-scale indoor-outdoor scenes, diverse human motions, rich human-human interactions, and human-environment interactions. By utilizing body-mounted IMUs and a head-mounted LiDAR, HiSC4D can capture egocentric human motions in unconstrained space without the need for external devices and pre-built maps. This affords great flexibility and accessibility for human-centered interaction and 4D scene capturing in various environments. Taking into account that IMUs can capture human spatially unrestricted poses but are prone to drifting for long-period using, and while LiDAR is stable for global localization but rough for local positions and orientations, HiSC4D employs a joint optimization method, harmonizing all sensors and utilizing environment cues, yielding promising results for long-term capture in large scenes. To promote research of egocentric human interaction in large scenes and facilitate downstream tasks, we also present a dataset, containing 8 sequences in 4 large scenes (200 to 5,000 $m^2$), providing 36k frames of accurate 4D human motions with SMPL annotations and dynamic scenes, 31k frames of cropped human point clouds, and scene mesh of the environment. A variety of scenarios, such as the basketball gym and commercial street, alongside challenging human motions, such as daily greeting, one-on-one basketball playing, and tour guiding, demonstrate the effectiveness and the generalization ability of HiSC4D. The dataset and code will be publicated on www.lidarhumanmotion.net/hisc4d available for research purposes.

==> tables/mpjpe.tex <==
\begin{table}[htb!]
	\centering
    \caption{Quantitative comparison of methods on HSC-LiDARCap. ($Ft.$): finetune on our data. ($Opt.$): optimized with our method. ($Sample.$): use the sampled data for mixed training.}
	\centering
    \begin{tabular}{l|lll}
        \toprule
        Method & \multicolumn{1}{l}{MPJPE} & \multicolumn{1}{l}{PA-MPJPE} & - \\
        \midrule
        LiDARCap &       &  &\\
        LiDARCap + $Ft.$ &   &  &\\
        LiDARCap + $Opt.$ &       &  &\\
        LiDARCap + $Ft.$ + $Opt.$ &       &  &\\
        \midrule
        Ours ($Sample.$ + $Ft.$ + $Opt.$) & 88.4  & 77.4 &\\
        \bottomrule
        \end{tabular}%
	\label{tab:mpjpe}
\end{table}

